Scalable Surface Reconstruction with Delaunay-Graph Neural Networks

We introduce a novel learning-based, visibility-aware, surface reconstruction method for large-scale, defect-laden point clouds. Our approach can cope with the scale and variety of point cloud defects encountered in real-life Multi-View Stereo (MVS) acquisitions. Our method relies on a 3D Delaunay tetrahedralization whose cells are classified as inside or outside the surface by a graph neural network and an energy model solvable with a graph cut. Our model, making use of both local geometric attributes and line-of-sight visibility information, is able to learn a visibility model from a small amount of synthetic training data and generalizes to real-life acquisitions. Combining the efficiency of deep learning methods and the scalability of energy based models, our approach outperforms both learning and non learning-based reconstruction algorithms on two publicly available reconstruction benchmarks. Our code and data is available at https://github.com/raphaelsulzer/dgnn.

==> 8_coverletter.tex <==
\twocolumn[{
\begin{center}
     \Huge \textbf{Revisions of SGP 2021 paper 1082}
\end{center}
~\\~\\
}]
We thank the reviewers for their thorough and insightful comments. We have taken into account their remarks and suggestions, and have highlighted our main changes in the text in \textcolor{red}{red}. In the following, we provide answers to the three points raised by the primary.

\noindent
\textbf{(a) Clarify the nature of the GraphSAGE-type learning formulation, and how it differs from standard techniques.}

We agree that our explanation of \secref{sec:contextual} was lacking in clarity, and we entirely rewrote it. After a careful rereading of the GraphSAGE paper, we agree with \RTHREE~that our custom implementation (with batch normalization after each iteration, allowing for node-wise inference) falls under the very general formulation of the original GraphSAGE paper. We have reworded all mentions of GraphSAGE to give proper credit.

\noindent
\textbf{(b) Present results after automatically filtering floating components, \eg as supported by the Poisson Reconstruction software
}

We thank \RFOUR~for suggesting the use of trimming for the Screened Poisson reconstruction. We have experimented with different trimming values, but could not find consistent parameters that improve the mean values of Poisson presented in \tabref{tab:berger} and \tabref{tab:results}. This is a problem that is mentioned by the authors of the Screened Poisson reconstruction themselves \cite[Sec.~1, p~2]{Kazhdan2020}. High trimming values remove valid surface parts in the low resolution scanner setting, which results in a surface that is no longer watertight. Conversely, low trimming values are not able to remove all floating components resulting from outliers.

Nonetheless, we were able to simultaneously address the floating artifacts and improve the overall results of the Poisson reconstruction by using the Dirichlet boundary condition for object-level reconstruction. Using this boundary condition, the indicator function is forced to be $-\frac{1}{2}$ on the bounding box of the object, which in practice prevents the reconstruction of floating artifacts near the bounding box. We have updated all corresponding figures and \tabref{tab:berger}. In open scene reconstruction evaluated with the ETH3D dataset, the bounding box is far away from the main scene due to sparsely captured background information. Changing the boundary condition of Screened Poisson does not influence the results in this case. We keep the Neumann boundary condition for this task, along with the post-processing step described in \secref{sec:clean}.
%Nonetheless, we have improved the results of the Poisson reconstruction by using the Dirichlet boundary condition for object-level reconstruction. Using this boundary condition, the indicator function is forced to be $-\frac{1}{2}$ on the bounding box of the object, which in practice prevents the reconstruction of floating artifacts near the bounding box. We have updated all corresponding figures and \tabref{tab:berger}. In open scene reconstruction evaluated with the ETH3D dataset, the bounding box is far away from the main scene due to sparsely captured background information. Changing the boundary condition of Screened Poisson does not influence the results here, thus, we keep the Neumann boundary condition for this task (and the post-processing step described in \secref{sec:clean}).

\noindent
\textbf{(c) Address typos and exposition problems throughout, and discuss limitations of the method.
}
We have corrected all typos and missing references kindly pointed out by the reviewers. We have added a discussion about the limitations of our model in \secref{sec:ablation}.

\balance
\pagebreak

==> tables/eth_accuracy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
% \resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l|cccc|cccc@{}}
\toprule
\multirow{2}{*}{} & \multicolumn{4}{c|}{\multirow{2}{*}{Accuracy - uncleaned}} & \multicolumn{4}{c}{\multirow{2}{*}{Accuracy - cleaned}} \\
 & \multicolumn{4}{c|}{} & \multicolumn{4}{c}{} \\
scene & Poisson & Vu et al. & Jan. et al. & Ours & Poisson & Vu et al. & Jan. et al. & Ours \\ \midrule
kicker & 0.67 & \textbf{0.77} & 0.69 & 0.73 & 0.68 & \textbf{0.80} & 0.76 & 0.79 \\
pipes & 0.82 & 0.80 & 0.76 & \textbf{0.88} & 0.84 & 0.82 & 0.80 & \textbf{0.92} \\
delivery\_area & 0.57 & 0.58 & 0.53 & \textbf{0.64} & 0.57 & 0.60 & 0.58 & \textbf{0.66} \\
meadow & 0.35 & 0.39 & 0.37 & \textbf{0.51} & 0.32 & 0.38 & 0.38 & \textbf{0.58} \\
office & 0.67 & 0.69 & 0.56 & \textbf{0.81} & 0.70 & 0.78 & 0.74 & \textbf{0.88} \\
playground & 0.51 & 0.63 & 0.54 & \textbf{0.65} & 0.50 & 0.66 & 0.60 & \textbf{0.73} \\
terrains & 0.65 & \textbf{0.74} & 0.71 & 0.69 & 0.66 & \textbf{0.76} & 0.75 & 0.73 \\
terrace & 0.75 & 0.68 & 0.66 & \textbf{0.83} & 0.77 & 0.74 & 0.73 & \textbf{0.88} \\
relief & 0.65 & 0.56 & 0.53 & \textbf{0.86} & 0.66 & 0.61 & 0.58 & \textbf{0.89} \\
relief\_2 & 0.63 & 0.58 & 0.56 & \textbf{0.85} & 0.64 & 0.64 & 0.63 & \textbf{0.88} \\
electro & 0.54 & 0.51 & 0.47 & \textbf{0.58} & 0.54 & 0.54 & 0.52 & \textbf{0.60} \\
courtyard & \textbf{0.72} & 0.67 & 0.62 & 0.69 & \textbf{0.73} & 0.69 & 0.68 & 0.72 \\
facade & 0.40 & 0.43 & 0.41 & \textbf{0.56} & 0.42 & 0.50 & 0.48 & \textbf{0.58} \\ \midrule
mean & 0.61 & 0.62 & 0.57 & \textbf{0.71} & 0.62 & 0.65 & 0.63 & \textbf{0.76} \\ \bottomrule
\end{tabular}%
% }
\caption{Accuracy of all scenes of the train dataset of ETH3D \cite{Schops2017} for uncleaned and cleaned mesh reconstructions at distance $\tau = 5$\,cm. The best (highest) values per scene are in bold letters. We perform better than all competing methods on 10 scenes out of 13. On average, we gain between 11 and 14\%. The mesh cleaning improves the accuracy of the reconstruction by 1 to 6\%.}
\label{tab:eth_accuracy}
\end{table*}

==> tables/eth_completeness.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
% \resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l|cccc|cccc@{}}
\toprule
\multirow{2}{*}{} & \multicolumn{4}{c|}{\multirow{2}{*}{Completeness - uncleaned}} & \multicolumn{4}{c}{\multirow{2}{*}{Completeness - cleaned}} \\
 & \multicolumn{4}{c|}{} & \multicolumn{4}{c}{} \\
scene & Poisson & Vu et al. & Jan. et al. & Ours & Poisson & Vu et al. & Jan. et al. & Ours \\ \midrule
kicker & \textbf{0.85} & 0.82 & 0.82 & 0.79 & \textbf{0.84} & 0.81 & 0.81 & 0.77 \\
pipes & 0.73 & \textbf{0.78} & \textbf{0.78} & 0.67 & 0.72 & \textbf{0.74} & \textbf{0.74} & 0.63 \\
delivery\_area & \textbf{0.88} & \textbf{0.88} & 0.87 & 0.80 & \textbf{0.87} & 0.84 & 0.84 & 0.77 \\
meadow & 0.64 & 0.76 & \textbf{0.78} & 0.68 & 0.53 & 0.74 & \textbf{0.76} & 0.63 \\
office & 0.54 & \textbf{0.62} & \textbf{0.62} & 0.47 & 0.53 & \textbf{0.54} & 0.53 & 0.43 \\
playground & \textbf{0.77} & \textbf{0.77} & 0.76 & 0.76 & \textbf{0.75} & 0.73 & 0.72 & 0.72 \\
terrains & \textbf{0.85} & 0.81 & 0.81 & 0.83 & \textbf{0.84} & 0.80 & 0.79 & 0.79 \\
terrace & 0.84 & \textbf{0.86} & \textbf{0.86} & 0.83 & 0.80 & \textbf{0.84} & \textbf{0.84} & 0.81 \\
relief & 0.81 & \textbf{0.83} & 0.82 & 0.75 & \textbf{0.80} & 0.79 & 0.79 & 0.73 \\
relief\_2 & 0.80 & \textbf{0.82} & \textbf{0.82} & 0.73 & \textbf{0.80} & 0.78 & 0.78 & 0.71 \\
electro & 0.83 & \textbf{0.84} & \textbf{0.84} & 0.83 & 0.82 & \textbf{0.83} & 0.82 & 0.81 \\
courtyard & 0.80 & 0.85 & 0.85 & \textbf{0.86} & 0.77 & \textbf{0.82} & \textbf{0.82} & \textbf{0.82} \\
facade & \textbf{0.67} & 0.66 & 0.66 & 0.50 & \textbf{0.65} & 0.61 & 0.61 & 0.44 \\ \midrule
mean & 0.77 & \textbf{0.79} & \textbf{0.79} & 0.73 & 0.75 & \textbf{0.76} & \textbf{0.76} & 0.70 \\ \bottomrule
\end{tabular}%
% }
\caption{Completeness of all scenes of the train dataset of ETH3D \cite{Schops2017} for uncleaned and cleaned mesh reconstructions at distance $\tau = 5$\,cm. The best (highest) values per scene are in bold letters. Screened poisson \cite{screened_poisson}, Vu \etal \cite{Vu2012} and Jancosek \etal \cite{Jancosek2014} perform better compared to our method on all scenes, except on \emph{courtyard}. On average we loose 6\% compared to Vu \etal and Jancosek \etal. The mesh cleaning also reduces the completeness of the reconstruction by 2 to 3\%.}
\label{tab:eth_completeness}
\end{table*}

==> tables/eth_results_cleaned.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
\toprule
 & \multicolumn{3}{c|}{\multirow{2}{*}{Poisson}} & \multicolumn{3}{c|}{\multirow{2}{*}{Vu et al.}} & \multicolumn{3}{c|}{\multirow{2}{*}{Jancosek et al.}} & \multicolumn{3}{c}{\multirow{2}{*}{Ours}} \\
 & \multicolumn{3}{c|}{} & \multicolumn{3}{c|}{} & \multicolumn{3}{c|}{} & \multicolumn{3}{c}{} \\ \midrule
scene & \multicolumn{1}{l}{Completen.} & \multicolumn{1}{l}{Accuracy} & \multicolumn{1}{l|}{F1-score} & \multicolumn{1}{l}{Completen.} & \multicolumn{1}{l}{Accuracy} & \multicolumn{1}{l|}{F1-score} & \multicolumn{1}{l}{Completen.} & \multicolumn{1}{l}{Accuracy} & \multicolumn{1}{l|}{F1-score} & \multicolumn{1}{l}{Completen.} & \multicolumn{1}{l}{Accuracy} & \multicolumn{1}{l}{F1-score} \\ \midrule
kicker & \textbf{0.85} & 0.67 & 0.75 & 0.81 & \textbf{0.80} & \textbf{0.81} & 0.81 & 0.76 & 0.78 & 0.77 & 0.79 & 0.78 \\
pipes & 0.73 & 0.82 & 0.77 & 0.74 & 0.82 & \textbf{0.78} & \textbf{0.74} & 0.80 & 0.77 & 0.63 & \textbf{0.92} & 0.75 \\
delivery area & \textbf{0.88} & 0.57 & 0.69 & 0.84 & 0.60 & 0.70 & 0.84 & 0.58 & 0.68 & 0.77 & \textbf{0.66} & \textbf{0.71} \\
meadow & 0.64 & 0.35 & 0.45 & 0.74 & 0.38 & 0.50 & \textbf{0.76} & 0.38 & 0.50 & 0.63 & \textbf{0.58} & \textbf{0.60} \\
office & 0.54 & 0.67 & 0.60 & \textbf{0.54} & 0.78 & \textbf{0.64} & 0.53 & 0.74 & 0.62 & 0.43 & \textbf{0.88} & 0.58 \\
playground & \textbf{0.77} & 0.51 & 0.61 & 0.73 & 0.66 & 0.69 & 0.72 & 0.60 & 0.66 & 0.72 & \textbf{0.73} & \textbf{0.73} \\
terrains & \textbf{0.85} & 0.65 & 0.73 & 0.80 & \textbf{0.76} & \textbf{0.78} & 0.79 & 0.75 & 0.77 & 0.79 & 0.73 & 0.76 \\
terrace & 0.84 & 0.75 & 0.79 & \textbf{0.84} & 0.74 & 0.79 & 0.84 & 0.73 & 0.78 & 0.81 & \textbf{0.88} & \textbf{0.85} \\
relief & \textbf{0.81} & 0.65 & 0.72 & 0.79 & 0.61 & 0.69 & 0.79 & 0.58 & 0.67 & 0.73 & \textbf{0.89} & \textbf{0.80} \\
relief 2 & \textbf{0.80} & 0.63 & 0.70 & 0.78 & 0.64 & 0.70 & \textbf{0.78} & 0.63 & 0.70 & 0.71 & \textbf{0.88} & \textbf{0.78} \\
electro & \textbf{0.83} & 0.54 & 0.65 & 0.83 & 0.54 & 0.65 & 0.82 & 0.52 & 0.64 & 0.81 & \textbf{0.60} & \textbf{0.69} \\
courtyard & 0.80 & 0.72 & 0.76 & 0.82 & 0.69 & 0.75 & 0.82 & 0.68 & 0.74 & \textbf{0.82} & \textbf{0.72} & \textbf{0.77} \\
facade & \textbf{0.67} & 0.40 & 0.50 & \textbf{0.61} & 0.50 & \textbf{0.55} & 0.61 & 0.48 & 0.54 & 0.44 & \textbf{0.58} & 0.50 \\ \midrule
mean & \textbf{0.77} & 0.61 & 0.67 & 0.76 & 0.65 & 0.69 & 0.76 & 0.63 & 0.68 & 0.70 & \textbf{0.76} & \textbf{0.71} \\ \bottomrule
\end{tabular}%
}
\caption{Results of all scenes of the train dataset of ETH3D \cite{Schops2017} for cleaned mesh reconstructions at distance $\tau = 5 cm$. The best (highest) values for Completeness (Completen.), Accuracy and F1-score per scene are in bold letters.}
\label{tab:eth_cleaned}
\end{table*}

==> tables/eth_results_uncleaned.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
\toprule
 & \multicolumn{3}{c|}{\multirow{2}{*}{Poisson}} & \multicolumn{3}{c|}{\multirow{2}{*}{Vu et al.}} & \multicolumn{3}{c|}{\multirow{2}{*}{Jancosek et al.}} & \multicolumn{3}{c}{\multirow{2}{*}{Ours}} \\
 & \multicolumn{3}{c|}{} & \multicolumn{3}{c|}{} & \multicolumn{3}{c|}{} & \multicolumn{3}{c}{} \\ \midrule
scene & \multicolumn{1}{l}{Completen.} & \multicolumn{1}{l}{Accuracy} & \multicolumn{1}{l|}{F1-score} & \multicolumn{1}{l}{Completen.} & \multicolumn{1}{l}{Accuracy} & \multicolumn{1}{l|}{F1-score} & \multicolumn{1}{l}{Completen.} & \multicolumn{1}{l}{Accuracy} & \multicolumn{1}{l|}{F1-score} & \multicolumn{1}{l}{Completen.} & \multicolumn{1}{l}{Accuracy} & \multicolumn{1}{l}{F1-score} \\ \midrule
kicker & \textbf{0.84} & 0.68 & 0.75 & 0.82 & \textbf{0.77} & \textbf{0.79} & 0.82 & 0.69 & 0.75 & 0.79 & 0.73 & 0.76 \\
pipes & 0.72 & 0.84 & 0.77 & 0.78 & 0.80 & \textbf{0.79} & \textbf{0.78} & 0.76 & 0.77 & 0.67 & \textbf{0.88} & 0.76 \\
delivery\_area & \textbf{0.87} & 0.57 & 0.69 & \textbf{0.88} & 0.58 & 0.70 & 0.87 & 0.53 & 0.66 & 0.80 & \textbf{0.64} & \textbf{0.71} \\
meadow & 0.53 & 0.32 & 0.40 & 0.76 & 0.39 & 0.52 & \textbf{0.78} & 0.37 & 0.51 & 0.68 & \textbf{0.51} & \textbf{0.58} \\
office & 0.53 & 0.70 & 0.60 & \textbf{0.62} & 0.69 & \textbf{0.65} & \textbf{0.62} & 0.56 & 0.59 & 0.47 & \textbf{0.81} & 0.59 \\
playground & \textbf{0.75} & 0.50 & 0.60 & \textbf{0.77} & 0.63 & 0.70 & 0.76 & 0.54 & 0.63 & 0.76 & \textbf{0.65} & \textbf{0.70} \\
terrains & \textbf{0.84} & 0.66 & 0.74 & 0.81 & \textbf{0.74} & \textbf{0.78} & 0.81 & 0.71 & 0.76 & 0.83 & 0.69 & 0.75 \\
terrace & 0.80 & 0.77 & 0.79 & \textbf{0.86} & 0.68 & 0.76 & 0.86 & 0.66 & 0.74 & 0.83 & \textbf{0.83} & \textbf{0.83} \\
relief & \textbf{0.80} & 0.66 & 0.73 & \textbf{0.83} & 0.56 & 0.67 & 0.82 & 0.53 & 0.64 & 0.75 & \textbf{0.86} & \textbf{0.80} \\
relief\_2 & \textbf{0.80} & 0.64 & 0.71 & \textbf{0.82} & 0.58 & 0.68 & \textbf{0.82} & 0.56 & 0.67 & 0.73 & \textbf{0.85} & \textbf{0.79} \\
electro & \textbf{0.82} & 0.54 & 0.65 & \textbf{0.84} & 0.51 & 0.64 & 0.84 & 0.47 & 0.60 & 0.83 & \textbf{0.58} & \textbf{0.68} \\
courtyard & 0.77 & \textbf{0.73} & 0.75 & 0.85 & 0.67 & 0.75 & 0.85 & 0.62 & 0.72 & \textbf{0.86} & \textbf{0.69} & \textbf{0.77} \\
facade & \textbf{0.65} & 0.42 & 0.51 & \textbf{0.66} & 0.43 & \textbf{0.52} & \textbf{0.66} & 0.41 & 0.50 & 0.50 & \textbf{0.56} & \textbf{0.53} \\ \midrule
mean & \textbf{0.75} & 0.62 & 0.67 & \textbf{0.79} & 0.62 & 0.69 & 0.79 & 0.57 & 0.66 & 0.73 & \textbf{0.71} & \textbf{0.71} \\ \bottomrule
\end{tabular}%
}
\caption{Results of all scenes of the train dataset of ETH3D \cite{Schops2017} for uncleaned mesh reconstructions at distance $\tau = 5 cm$. The best (highest) values for Completeness (Completen.), Accuracy and F1-score per scene are in bold letters.}
\label{tab:eth_uncleaned}
\end{table*}

==> tables/supp_cleaned.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c }
\hline
 & \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{3}{c}{\cellcolor[HTML]{FFFFFF}} \\
 & \multicolumn{3}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}Vu \textit{et al.} \cite{Vu2012}}} & \multicolumn{3}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}Jancosek \textit{et al.} \cite{Jancosek2014}}} & \multicolumn{3}{c}{\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}Ours}} \\
scene & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}Completen.} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}Accuracy} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}F1-score} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}Completen.} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}Accuracy} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}F1-score} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}Completen.} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}Accuracy} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}F1-score} \\ \hline
kicker & \textbf{0.81} & \textbf{0.80} & \textbf{0.81} & 0.81 & 0.76 & 0.78 & 0.77 & 0.79 & 0.78 \\
pipes & 0.74 & 0.82 & \textbf{0.78} & \textbf{0.74} & 0.80 & 0.77 & 0.63 & \textbf{0.92} & 0.75 \\
delivery\_area & \textbf{0.84} & \textbf{0.60} & 0.70 & 0.84 & 0.58 & 0.68 & 0.77 & \textbf{0.66} & \textbf{0.71} \\
meadow & 0.74 & 0.38 & 0.50 & \textbf{0.76} & 0.38 & 0.50 & 0.63 & \textbf{0.58} & \textbf{0.60} \\
office & \textbf{0.54} & 0.78 & \textbf{0.64} & 0.53 & 0.74 & 0.62 & 0.43 & \textbf{0.88} & 0.58 \\
playground & \textbf{0.73} & 0.66 & 0.69 & 0.72 & 0.60 & 0.66 & 0.72 & \textbf{0.73} & \textbf{0.73} \\
terrains & \textbf{0.80} & \textbf{0.76} & \textbf{0.78} & 0.79 & 0.75 & 0.77 & 0.79 & 0.73 & 0.76 \\
terrace & \textbf{0.84} & 0.74 & 0.79 & 0.84 & 0.73 & 0.78 & 0.81 & \textbf{0.88} & \textbf{0.85} \\
relief & \textbf{0.79} & 0.61 & 0.69 & 0.79 & 0.58 & 0.67 & 0.73 & \textbf{0.89} & \textbf{0.80} \\
relief\_2 & 0.78 & 0.64 & 0.70 & \textbf{0.78} & 0.63 & 0.70 & 0.71 & \textbf{0.88} & \textbf{0.78} \\
electro & \textbf{0.83} & 0.54 & 0.65 & 0.82 & 0.52 & 0.64 & 0.81 & \textbf{0.60} & \textbf{0.69} \\
courtyard & 0.82 & 0.69 & 0.75 & 0.82 & 0.68 & 0.74 & \textbf{0.82} & \textbf{0.72} & \textbf{0.77} \\
facade & \textbf{0.61} & 0.50 & \textbf{0.55} & 0.61 & 0.48 & 0.54 & 0.44 & \textbf{0.58} & 0.50 \\ \hline
mean & \textbf{0.759} & 0.653 & 0.693 & 0.759 & 0.633 & 0.681 & 0.696 & \textbf{0.757} & \textbf{0.714} \\ \hline
\end{tabular}%
}
\caption{Results of all scenes of the train dataset of ETH3D \cite{Schops2017} for cleaned mesh reconstructions at distance $\tau = 5 cm$. The best (highest) values for Completeness (Completen.), Accuracy and F1-score per scene are in bold letters.}
\label{tab:supp_cleaned}
\end{table*}

==> tables/supp_uncleaned.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c }
\hline
 & \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{3}{c}{\cellcolor[HTML]{FFFFFF}} \\
 & \multicolumn{3}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}Vu \textit{et al.} \cite{Vu2012}}} & \multicolumn{3}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}Jancosek \textit{et al.} \cite{Jancosek2014}}} & \multicolumn{3}{c}{\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}Ours}} \\
scene & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}Completen.} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}Accuracy} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}F1-score} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}Completen.} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}Accuracy} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}F1-score} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}Completen.} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}Accuracy} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}F1-score} \\ \hline
kicker & \textbf{0.82} & \textbf{0.77} & \textbf{0.79} & 0.82 & 0.69 & 0.75 & 0.79 & 0.73 & 0.76 \\
pipes & 0.78 & 0.80 & \textbf{0.79} & \textbf{0.78} & 0.76 & 0.77 & 0.67 & \textbf{0.88} & 0.76 \\
delivery\_area & \textbf{0.88} & 0.58 & 0.70 & 0.87 & 0.53 & 0.66 & 0.80 & \textbf{0.64} & \textbf{0.71} \\
meadow & 0.76 & 0.39 & 0.52 & \textbf{0.78} & 0.37 & 0.51 & 0.68 & \textbf{0.51} & \textbf{0.58} \\
office & 0.62 & 0.69 & \textbf{0.65} & \textbf{0.62} & 0.56 & 0.59 & 0.47 & \textbf{0.81} & 0.59 \\
playground & \textbf{0.77} & 0.63 & 0.70 & 0.76 & 0.54 & 0.63 & 0.76 & \textbf{0.65} & \textbf{0.70} \\
terrains & 0.81 & \textbf{0.74} & \textbf{0.78} & 0.81 & 0.71 & 0.76 & \textbf{0.83} & 0.69 & 0.75 \\
terrace & \textbf{0.86} & 0.68 & 0.76 & 0.86 & 0.66 & 0.74 & 0.83 & \textbf{0.83} & \textbf{0.83} \\
relief & \textbf{0.83} & 0.56 & 0.67 & 0.82 & 0.53 & 0.64 & 0.75 & \textbf{0.86} & \textbf{0.80} \\
relief\_2 & \textbf{0.82} & 0.58 & 0.68 & 0.82 & 0.56 & 0.67 & 0.73 & \textbf{0.85} & \textbf{0.79} \\
electro & \textbf{0.84} & 0.51 & 0.64 & 0.84 & 0.47 & 0.60 & 0.83 & \textbf{0.58} & \textbf{0.68} \\
courtyard & 0.85 & 0.67 & 0.75 & 0.85 & 0.62 & 0.72 & \textbf{0.86} & \textbf{0.69} & \textbf{0.77} \\
facade & 0.66 & 0.43 & 0.52 & \textbf{0.66} & 0.41 & 0.50 & 0.50 & \textbf{0.56} & \textbf{0.53} \\ \hline
mean & \textbf{0.793} & 0.619 & 0.688 & 0.793 & 0.569 & 0.657 & 0.731 & \textbf{0.714} & \textbf{0.712} \\ \hline
\end{tabular}%
}
\caption{Results of all scenes of the train dataset of ETH3D \cite{Schops2017} for uncleaned mesh reconstructions at distance $\tau = 5 cm$. The best (highest) values for Completeness (Completen.), Accuracy and F1-score per scene are in bold letters.}
\label{tab:supp_uncleaned}
\end{table*}
